A General Destriping Framework for Remote Sensing Images Using Flatness Constraint

Removing stripe noise, i.e., destriping, from remote sensing images is an essential task in terms of visual quality and subsequent processing. Most existing destriping methods are designed by combining a particular image regularization with a stripe noise characterization that cooperates with the regularization, which precludes us to examine and activate different regularizations to adapt to various target images. To resolve this, two requirements need to be considered: a general framework that can handle a variety of image regularizations in destriping, and a strong stripe noise characterization that can consistently capture the nature of stripe noise, regardless of the choice of image regularization. To this end, this paper proposes a general destriping framework using a newly-introduced stripe noise characterization, named flatness constraint, where we can handle various regularization functions in a unified manner. Specifically, we formulate the destriping problem as a nonsmooth convex optimization problem involving a general form of image regularization and the flatness constraint. The constraint mathematically models that the intensity of each stripe is constant along one direction, resulting in a strong characterization of stripe noise. For solving the optimization problem, we also develop an efficient algorithm based on a diagonally preconditioned primal-dual splitting algorithm (DP-PDS), which can automatically adjust the stepsizes. The effectiveness of our framework is demonstrated through destriping experiments, where we comprehensively compare combinations of a variety of image regularizations and stripe noise characterizations using hyperspectral images (HSI) and infrared (IR) videos.

==> fig_tex/fig_SSTV_mo_spe_sig.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/SSTV_Mo_so_spe_sig_150_80.eps}}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/SSTV_Mo_so_spe_sig_157_23.eps}}
	\end{minipage}
	
	
	\begin{minipage}{0.49\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{(b)}
	\end{minipage}

	\caption{The spectral signature of the destriping results in Case (i) with SSTV. (a): The green field area. (b): The boundary between green field area and river.}
	\label{fig:SSTV_mo_spe_sig}
\end{figure}

==> fig_tex/fig_TNN_sa_spe_sig.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/TNN_Sa_sg_spe_sig_200_40.eps}}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/TNN_Sa_sg_spe_sig_242_47.eps}}
	\end{minipage}
	
	
	\begin{minipage}{0.49\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{(b)}
	\end{minipage}

	\caption{The spectral signature of the destriping results in Case (iii) with TNN. (a): The green field area. (b): The house area.}
	\label{fig:TNN_sa_spe_sig}
\end{figure}

==> fig_tex/fig_bw_PSNR_SSIM_ATV.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_IR_destriping/ATV_test2_PSNR.eps}}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_IR_destriping/ATV_test2_SSIM.eps}}
	\end{minipage}
	
	
	\begin{minipage}{0.49\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{(b)}
	\end{minipage}
	
	\caption{Band-wise PSNRs and SSIMs of the \textit{Birds1} destriping results in Case (ii) using ATV.}
	\label{fig:bw_PSNR_SSIM_ATV}
\end{figure}

==> fig_tex/fig_bw_PSNR_SSIM_SSTV.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/SSTV_Mo_so_PSNR.eps}}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/SSTV_Mo_so_SSIM.eps}}
	\end{minipage}
	
	\begin{minipage}{0.49\hsize}
		\centerline{(a)}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{(b)}
	\end{minipage}
	
	\caption{Band-wise PSNRs and SSIMs of the \textit{Moffett field} destriping results in Case (i) using SSTV.}
	\label{fig:bw_PSNR_SSIM_SSTV}
\end{figure}

==> fig_tex/fig_bw_PSNR_SSIM_TNN.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/TNN_Sa_sg_PSNR.eps}}
	\end{minipage}
	\begin{minipage}{0.49\hsize}
		\centerline{\includegraphics[width=\hsize]{./fig/result_HSI_destriping/TNN_Sa_sg_SSIM.eps}}
	\end{minipage}
	
	\caption{Band-wise PSNRs and SSIMs of the \textit{Salinas} destriping results in Case (iii) using TNN.}
	\label{fig:bw_PSNR_SSIM_TNN}
\end{figure}

==> table_latex/tab_PSNR_and_SSIM_spe_sig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PSNR, SSIM and time of simulated destriping results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
	\begin{center}
		\caption{MPSNR and MSSIM of the HSI Destriping Results in Case (iv)}
		\label{tab:PSNR_and_SSIM_spe_sig}
		%		\begin{tabular}{|c|c|c|cc|c|c|cc|c|c|c|c|}
		\begin{tabular}{ccccccccccccc}
			\toprule
			\multirow{2}{*}{Image data} & range of & Regularization & \multicolumn{5}{c}{MPSNR} & \multicolumn{5}{c}{MSSIM} \\
			\cmidrule(lr){4-8} 
			\cmidrule(lr){9-13}
			& stripe noise & function & S~\cite{LRMR} & GS~\cite{GLSSTV} & LR~\cite{NN_char} & TV~\cite{gradient_constraint} & FC & S~\cite{LRMR} & GS~\cite{GLSSTV} & LR~\cite{NN_char} & TV~\cite{gradient_constraint} & FC \\ 
			\midrule
			&
			\multirow{5}{*}{$[-0.3,0.3]$} 
			& HTV
			& \textcolor{red}{\textbf{27.80}} & \textcolor{blue}{\textbf{29.03}} & \textcolor{red}{28.33} & \textcolor{blue}{28.95} & \textcolor{blue}{28.95} &
			\textcolor{red}{\textbf{0.8130}} & \textcolor{blue}{\textbf{0.8811}} & \textcolor{red}{0.8488} & \textcolor{blue}{0.8741} & \textcolor{blue}{0.8741} \\
			& & SSTV
			& \textcolor{blue}{30.87} & \textcolor{blue}{\textbf{30.90}} & 30.76 & \textcolor{red}{30.50} & \textcolor{red}{30.50} &
			\textcolor{blue}{0.9640} & \textcolor{blue}{\textbf{0.9656}} & 0.9631 & \textcolor{red}{0.9415} & \textcolor{red}{0.9415} \\
			& & ASSTV
			& \textcolor{red}{\textbf{30.70}} & \textcolor{blue}{\textbf{31.31}} & \textcolor{blue}{31.23} & \textcolor{red}{30.98} & 31.01 &
			\textcolor{red}{0.9385} & \textcolor{blue}{\textbf{0.9604}} & \textcolor{blue}{0.9594} & \textcolor{red}{\textbf{0.9378}} & 0.9390 \\
			& & TNN
			& \textcolor{red}{\textbf{26.40}} & \textcolor{red}{29.54} & 30.85 & \textcolor{blue}{\textbf{31.66}} & \textcolor{blue}{\textbf{31.66}} &
			\textcolor{red}{\textbf{0.7491}} & \textcolor{red}{0.8802} & 0.9203 & \textcolor{blue}{\textbf{0.9224}} & \textcolor{blue}{\textbf{0.9224}} \\
			& & SSTV+TNN
			& \textcolor{red}{30.48} & \textcolor{blue}{31.17} & \textcolor{blue}{\textbf{31.27}} & 30.52 & \textcolor{red}{\textbf{30.26}} &
			0.9314 & \textcolor{blue}{0.9582} & \textcolor{blue}{\textbf{0.9601}} & \textcolor{red}{0.9169} & \textcolor{red}{\textbf{0.9123}} \\
			& & $l_{0}$-$l_{1}$HTV
			& \textcolor{red}{\textbf{30.54}} & \textcolor{blue}{\textbf{30.99}} & \textcolor{blue}{30.95} & 30.65 & 30.65 &
			\textcolor{red}{\textbf{0.9438}} & \textcolor{blue}{0.9618} & \textcolor{blue}{\textbf{0.9619}} & 0.9453 & 0.9453 \\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table*}
